Study of the decay $J/\psi \to \phi \pi^{0}\eta$

Based on $(10.09 \pm 0.04) \times 10^9$ $J/\psi$ events collected with the BESIII detector operating at the BEPCII collider, a partial wave analysis of the decay $J/\psi \to \phi \pi^{0}\eta$ is performed. We observe for the first time two new structures on the $\phi\eta$ invariant mass distribution, with statistical significances of $24.0\sigma$ and $16.9\sigma$; the first with $J^{\rm PC}$ = $1^{+-}$, mass M = (1911 $\pm$ 6 (stat.) $\pm$ 14 (sys.))~MeV/$c^{2}$, and width $\Gamma = $ (149 $\pm$ 12 (stat.) $\pm$ 23 (sys.))~MeV, the second with $J^{\rm PC}$ = $1^{--}$, mass M = (1996 $\pm$ 11 (stat.) $\pm$ 30 (sys.))~MeV/$c^{2}$, and width $\Gamma$ = (148 $\pm$ 16 (stat.) $\pm$ 66 (sys.))~MeV. These measurements provide important input for the strangeonium spectrum. In addition, the $f_0(980)-a_0(980)^0$ mixing signal in $J/\psi \to \phi f_0(980) \to \phi a_0(980)^0$ and the corresponding electromagnetic decay $J/\psi \to \phi a_0(980)^0$ are measured with improved precision, providing crucial information to understand the nature of $a_0(980)^0$ and $f_0(980)$.

==> authors.tex <==
\author{
\begin{small}
\begin{center}
%% Saved at => 2023-08-14
M.~Ablikim$^{1}$, M.~N.~Achasov$^{4,b}$, P.~Adlarson$^{75}$, X.~C.~Ai$^{80}$, R.~Aliberti$^{35}$, A.~Amoroso$^{74A,74C}$, M.~R.~An$^{39}$, Q.~An$^{71,58}$, Y.~Bai$^{57}$, O.~Bakina$^{36}$, I.~Balossino$^{29A}$, Y.~Ban$^{46,g}$, H.-R.~Bao$^{63}$, V.~Batozskaya$^{1,44}$, K.~Begzsuren$^{32}$, N.~Berger$^{35}$, M.~Berlowski$^{44}$, M.~Bertani$^{28A}$, D.~Bettoni$^{29A}$, F.~Bianchi$^{74A,74C}$, E.~Bianco$^{74A,74C}$, A.~Bortone$^{74A,74C}$, I.~Boyko$^{36}$, R.~A.~Briere$^{5}$, A.~Brueggemann$^{68}$, H.~Cai$^{76}$, X.~Cai$^{1,58}$, A.~Calcaterra$^{28A}$, G.~F.~Cao$^{1,63}$, N.~Cao$^{1,63}$, S.~A.~Cetin$^{62A}$, J.~F.~Chang$^{1,58}$, W.~L.~Chang$^{1,63}$, G.~R.~Che$^{43}$, G.~Chelkov$^{36,a}$, C.~Chen$^{43}$, Chao~Chen$^{55}$, G.~Chen$^{1}$, H.~S.~Chen$^{1,63}$, M.~L.~Chen$^{1,58,63}$, S.~J.~Chen$^{42}$, S.~L.~Chen$^{45}$, S.~M.~Chen$^{61}$, T.~Chen$^{1,63}$, X.~R.~Chen$^{31,63}$, X.~T.~Chen$^{1,63}$, Y.~B.~Chen$^{1,58}$, Y.~Q.~Chen$^{34}$, Z.~J.~Chen$^{25,h}$, S.~K.~Choi$^{10A}$, X.~Chu$^{43}$, G.~Cibinetto$^{29A}$, S.~C.~Coen$^{3}$, F.~Cossio$^{74C}$, J.~J.~Cui$^{50}$, H.~L.~Dai$^{1,58}$, J.~P.~Dai$^{78}$, A.~Dbeyssi$^{18}$, R.~ E.~de Boer$^{3}$, D.~Dedovich$^{36}$, Z.~Y.~Deng$^{1}$, A.~Denig$^{35}$, I.~Denysenko$^{36}$, M.~Destefanis$^{74A,74C}$, F.~De~Mori$^{74A,74C}$, B.~Ding$^{66,1}$, X.~X.~Ding$^{46,g}$, Y.~Ding$^{34}$, Y.~Ding$^{40}$, J.~Dong$^{1,58}$, L.~Y.~Dong$^{1,63}$, M.~Y.~Dong$^{1,58,63}$, X.~Dong$^{76}$, M.~C.~Du$^{1}$, S.~X.~Du$^{80}$, Z.~H.~Duan$^{42}$, P.~Egorov$^{36,a}$, Y.~H.~Fan$^{45}$, J.~Fang$^{1,58}$, S.~S.~Fang$^{1,63}$, W.~X.~Fang$^{1}$, Y.~Fang$^{1}$, Y.~Q.~Fang$^{1,58}$, R.~Farinelli$^{29A}$, L.~Fava$^{74B,74C}$, F.~Feldbauer$^{3}$, G.~Felici$^{28A}$, C.~Q.~Feng$^{71,58}$, J.~H.~Feng$^{59}$, Y.~T.~Feng$^{71,58}$, K~Fischer$^{69}$, M.~Fritsch$^{3}$, C.~D.~Fu$^{1}$, J.~L.~Fu$^{63}$, Y.~W.~Fu$^{1}$, H.~Gao$^{63}$, Y.~N.~Gao$^{46,g}$, Yang~Gao$^{71,58}$, S.~Garbolino$^{74C}$, I.~Garzia$^{29A,29B}$, P.~T.~Ge$^{76}$, Z.~W.~Ge$^{42}$, C.~Geng$^{59}$, E.~M.~Gersabeck$^{67}$, A~Gilman$^{69}$, K.~Goetzen$^{13}$, L.~Gong$^{40}$, W.~X.~Gong$^{1,58}$, W.~Gradl$^{35}$, S.~Gramigna$^{29A,29B}$, M.~Greco$^{74A,74C}$, M.~H.~Gu$^{1,58}$, Y.~T.~Gu$^{15}$, C.~Y~Guan$^{1,63}$, Z.~L.~Guan$^{22}$, A.~Q.~Guo$^{31,63}$, L.~B.~Guo$^{41}$, M.~J.~Guo$^{50}$, R.~P.~Guo$^{49}$, Y.~P.~Guo$^{12,f}$, A.~Guskov$^{36,a}$, J.~Gutierrez$^{27}$, K.~L.~Han$^{63}$, T.~T.~Han$^{1}$, W.~Y.~Han$^{39}$, X.~Q.~Hao$^{19}$, F.~A.~Harris$^{65}$, K.~K.~He$^{55}$, K.~L.~He$^{1,63}$, F.~H~H..~Heinsius$^{3}$, C.~H.~Heinz$^{35}$, Y.~K.~Heng$^{1,58,63}$, C.~Herold$^{60}$, T.~Holtmann$^{3}$, P.~C.~Hong$^{12,f}$, G.~Y.~Hou$^{1,63}$, X.~T.~Hou$^{1,63}$, Y.~R.~Hou$^{63}$, Z.~L.~Hou$^{1}$, B.~Y.~Hu$^{59}$, H.~M.~Hu$^{1,63}$, J.~F.~Hu$^{56,i}$, T.~Hu$^{1,58,63}$, Y.~Hu$^{1}$, G.~S.~Huang$^{71,58}$, K.~X.~Huang$^{59}$, L.~Q.~Huang$^{31,63}$, X.~T.~Huang$^{50}$, Y.~P.~Huang$^{1}$, T.~Hussain$^{73}$, N~H\"usken$^{27,35}$, N.~in der Wiesche$^{68}$, M.~Irshad$^{71,58}$, J.~Jackson$^{27}$, S.~Jaeger$^{3}$, S.~Janchiv$^{32}$, J.~H.~Jeong$^{10A}$, Q.~Ji$^{1}$, Q.~P.~Ji$^{19}$, X.~B.~Ji$^{1,63}$, X.~L.~Ji$^{1,58}$, Y.~Y.~Ji$^{50}$, X.~Q.~Jia$^{50}$, Z.~K.~Jia$^{71,58}$, H.~B.~Jiang$^{76}$, P.~C.~Jiang$^{46,g}$, S.~S.~Jiang$^{39}$, T.~J.~Jiang$^{16}$, X.~S.~Jiang$^{1,58,63}$, Y.~Jiang$^{63}$, J.~B.~Jiao$^{50}$, Z.~Jiao$^{23}$, S.~Jin$^{42}$, Y.~Jin$^{66}$, M.~Q.~Jing$^{1,63}$, X.~M.~Jing$^{63}$, T.~Johansson$^{75}$, X.~K.$^{1}$, S.~Kabana$^{33}$, N.~Kalantar-Nayestanaki$^{64}$, X.~L.~Kang$^{9}$, X.~S.~Kang$^{40}$, M.~Kavatsyuk$^{64}$, B.~C.~Ke$^{80}$, V.~Khachatryan$^{27}$, A.~Khoukaz$^{68}$, R.~Kiuchi$^{1}$, O.~B.~Kolcu$^{62A}$, B.~Kopf$^{3}$, M.~Kuessner$^{3}$, A.~Kupsc$^{44,75}$, W.~K\"uhn$^{37}$, J.~J.~Lane$^{67}$, P. ~Larin$^{18}$, L.~Lavezzi$^{74A,74C}$, T.~T.~Lei$^{71,58}$, Z.~H.~Lei$^{71,58}$, H.~Leithoff$^{35}$, M.~Lellmann$^{35}$, T.~Lenz$^{35}$, C.~Li$^{43}$, C.~Li$^{47}$, C.~H.~Li$^{39}$, Cheng~Li$^{71,58}$, D.~M.~Li$^{80}$, F.~Li$^{1,58}$, G.~Li$^{1}$, H.~Li$^{71,58}$, H.~B.~Li$^{1,63}$, H.~J.~Li$^{19}$, H.~N.~Li$^{56,i}$, Hui~Li$^{43}$, J.~R.~Li$^{61}$, J.~S.~Li$^{59}$, J.~W.~Li$^{50}$, Ke~Li$^{1}$, L.~J~Li$^{1,63}$, L.~K.~Li$^{1}$, Lei~Li$^{48}$, M.~H.~Li$^{43}$, P.~R.~Li$^{38,k}$, Q.~X.~Li$^{50}$, S.~X.~Li$^{12}$, T. ~Li$^{50}$, W.~D.~Li$^{1,63}$, W.~G.~Li$^{1}$, X.~H.~Li$^{71,58}$, X.~L.~Li$^{50}$, Xiaoyu~Li$^{1,63}$, Y.~G.~Li$^{46,g}$, Z.~J.~Li$^{59}$, Z.~X.~Li$^{15}$, C.~Liang$^{42}$, H.~Liang$^{71,58}$, H.~Liang$^{1,63}$, Y.~F.~Liang$^{54}$, Y.~T.~Liang$^{31,63}$, G.~R.~Liao$^{14}$, L.~Z.~Liao$^{50}$, Y.~P.~Liao$^{1,63}$, J.~Libby$^{26}$, A. ~Limphirat$^{60}$, D.~X.~Lin$^{31,63}$, T.~Lin$^{1}$, B.~J.~Liu$^{1}$, B.~X.~Liu$^{76}$, C.~Liu$^{34}$, C.~X.~Liu$^{1}$, F.~H.~Liu$^{53}$, Fang~Liu$^{1}$, Feng~Liu$^{6}$, G.~M.~Liu$^{56,i}$, H.~Liu$^{38,j,k}$, H.~B.~Liu$^{15}$, H.~M.~Liu$^{1,63}$, Huanhuan~Liu$^{1}$, Huihui~Liu$^{21}$, J.~B.~Liu$^{71,58}$, J.~Y.~Liu$^{1,63}$, K.~Liu$^{38,j,k}$, K.~Y.~Liu$^{40}$, Ke~Liu$^{22}$, L.~Liu$^{71,58}$, L.~C.~Liu$^{43}$, Lu~Liu$^{43}$, M.~H.~Liu$^{12,f}$, P.~L.~Liu$^{1}$, Q.~Liu$^{63}$, S.~B.~Liu$^{71,58}$, T.~Liu$^{12,f}$, W.~K.~Liu$^{43}$, W.~M.~Liu$^{71,58}$, X.~Liu$^{38,j,k}$, Y.~Liu$^{38,j,k}$, Y.~Liu$^{80}$, Y.~B.~Liu$^{43}$, Z.~A.~Liu$^{1,58,63}$, Z.~Q.~Liu$^{50}$, X.~C.~Lou$^{1,58,63}$, F.~X.~Lu$^{59}$, H.~J.~Lu$^{23}$, J.~G.~Lu$^{1,58}$, X.~L.~Lu$^{1}$, Y.~Lu$^{7}$, Y.~P.~Lu$^{1,58}$, Z.~H.~Lu$^{1,63}$, C.~L.~Luo$^{41}$, M.~X.~Luo$^{79}$, T.~Luo$^{12,f}$, X.~L.~Luo$^{1,58}$, X.~R.~Lyu$^{63}$, Y.~F.~Lyu$^{43}$, F.~C.~Ma$^{40}$, H.~Ma$^{78}$, H.~L.~Ma$^{1}$, J.~L.~Ma$^{1,63}$, L.~L.~Ma$^{50}$, M.~M.~Ma$^{1,63}$, Q.~M.~Ma$^{1}$, R.~Q.~Ma$^{1,63}$, X.~Y.~Ma$^{1,58}$, Y.~Ma$^{46,g}$, Y.~M.~Ma$^{31}$, F.~E.~Maas$^{18}$, M.~Maggiora$^{74A,74C}$, S.~Malde$^{69}$, A.~Mangoni$^{28B}$, Y.~J.~Mao$^{46,g}$, Z.~P.~Mao$^{1}$, S.~Marcello$^{74A,74C}$, Z.~X.~Meng$^{66}$, J.~G.~Messchendorp$^{13,64}$, G.~Mezzadri$^{29A}$, H.~Miao$^{1,63}$, T.~J.~Min$^{42}$, R.~E.~Mitchell$^{27}$, X.~H.~Mo$^{1,58,63}$, B.~Moses$^{27}$, N.~Yu.~Muchnoi$^{4,b}$, J.~Muskalla$^{35}$, Y.~Nefedov$^{36}$, F.~Nerling$^{18,d}$, I.~B.~Nikolaev$^{4,b}$, Z.~Ning$^{1,58}$, S.~Nisar$^{11,l}$, Q.~L.~Niu$^{38,j,k}$, W.~D.~Niu$^{55}$, Y.~Niu $^{50}$, S.~L.~Olsen$^{63}$, Q.~Ouyang$^{1,58,63}$, S.~Pacetti$^{28B,28C}$, X.~Pan$^{55}$, Y.~Pan$^{57}$, A.~~Pathak$^{34}$, P.~Patteri$^{28A}$, Y.~P.~Pei$^{71,58}$, M.~Pelizaeus$^{3}$, H.~P.~Peng$^{71,58}$, Y.~Y.~Peng$^{38,j,k}$, K.~Peters$^{13,d}$, J.~L.~Ping$^{41}$, R.~G.~Ping$^{1,63}$, S.~Plura$^{35}$, V.~Prasad$^{33}$, F.~Z.~Qi$^{1}$, H.~Qi$^{71,58}$, H.~R.~Qi$^{61}$, M.~Qi$^{42}$, T.~Y.~Qi$^{12,f}$, S.~Qian$^{1,58}$, W.~B.~Qian$^{63}$, C.~F.~Qiao$^{63}$, J.~J.~Qin$^{72}$, L.~Q.~Qin$^{14}$, X.~S.~Qin$^{50}$, Z.~H.~Qin$^{1,58}$, J.~F.~Qiu$^{1}$, S.~Q.~Qu$^{61}$, C.~F.~Redmer$^{35}$, K.~J.~Ren$^{39}$, A.~Rivetti$^{74C}$, M.~Rolo$^{74C}$, G.~Rong$^{1,63}$, Ch.~Rosner$^{18}$, S.~N.~Ruan$^{43}$, N.~Salone$^{44}$, A.~Sarantsev$^{36,c}$, Y.~Schelhaas$^{35}$, K.~Schoenning$^{75}$, M.~Scodeggio$^{29A,29B}$, K.~Y.~Shan$^{12,f}$, W.~Shan$^{24}$, X.~Y.~Shan$^{71,58}$, J.~F.~Shangguan$^{55}$, L.~G.~Shao$^{1,63}$, M.~Shao$^{71,58}$, C.~P.~Shen$^{12,f}$, H.~F.~Shen$^{1,63}$, W.~H.~Shen$^{63}$, X.~Y.~Shen$^{1,63}$, B.~A.~Shi$^{63}$, H.~C.~Shi$^{71,58}$, J.~L.~Shi$^{12}$, J.~Y.~Shi$^{1}$, Q.~Q.~Shi$^{55}$, R.~S.~Shi$^{1,63}$, X.~Shi$^{1,58}$, J.~J.~Song$^{19}$, T.~Z.~Song$^{59}$, W.~M.~Song$^{34,1}$, Y. ~J.~Song$^{12}$, S.~Sosio$^{74A,74C}$, S.~Spataro$^{74A,74C}$, F.~Stieler$^{35}$, Y.~J.~Su$^{63}$, G.~B.~Sun$^{76}$, G.~X.~Sun$^{1}$, H.~Sun$^{63}$, H.~K.~Sun$^{1}$, J.~F.~Sun$^{19}$, K.~Sun$^{61}$, L.~Sun$^{76}$, S.~S.~Sun$^{1,63}$, T.~Sun$^{51,e}$, W.~Y.~Sun$^{34}$, Y.~Sun$^{9}$, Y.~J.~Sun$^{71,58}$, Y.~Z.~Sun$^{1}$, Z.~T.~Sun$^{50}$, Y.~X.~Tan$^{71,58}$, C.~J.~Tang$^{54}$, G.~Y.~Tang$^{1}$, J.~Tang$^{59}$, Y.~A.~Tang$^{76}$, L.~Y~Tao$^{72}$, Q.~T.~Tao$^{25,h}$, M.~Tat$^{69}$, J.~X.~Teng$^{71,58}$, V.~Thoren$^{75}$, W.~H.~Tian$^{52}$, W.~H.~Tian$^{59}$, Y.~Tian$^{31,63}$, Z.~F.~Tian$^{76}$, I.~Uman$^{62B}$, Y.~Wan$^{55}$,  S.~J.~Wang $^{50}$, B.~Wang$^{1}$, B.~L.~Wang$^{63}$, Bo~Wang$^{71,58}$, C.~W.~Wang$^{42}$, D.~Y.~Wang$^{46,g}$, F.~Wang$^{72}$, H.~J.~Wang$^{38,j,k}$, J.~P.~Wang $^{50}$, K.~Wang$^{1,58}$, L.~L.~Wang$^{1}$, M.~Wang$^{50}$, Meng~Wang$^{1,63}$, N.~Y.~Wang$^{63}$, S.~Wang$^{12,f}$, S.~Wang$^{38,j,k}$, T. ~Wang$^{12,f}$, T.~J.~Wang$^{43}$, W.~Wang$^{59}$, W. ~Wang$^{72}$, W.~P.~Wang$^{71,58}$, X.~Wang$^{46,g}$, X.~F.~Wang$^{38,j,k}$, X.~J.~Wang$^{39}$, X.~L.~Wang$^{12,f}$, Y.~Wang$^{61}$, Y.~D.~Wang$^{45}$, Y.~F.~Wang$^{1,58,63}$, Y.~L.~Wang$^{19}$, Y.~N.~Wang$^{45}$, Y.~Q.~Wang$^{1}$, Yaqian~Wang$^{17,1}$, Yi~Wang$^{61}$, Z.~Wang$^{1,58}$, Z.~L. ~Wang$^{72}$, Z.~Y.~Wang$^{1,63}$, Ziyi~Wang$^{63}$, D.~Wei$^{70}$, D.~H.~Wei$^{14}$, F.~Weidner$^{68}$, S.~P.~Wen$^{1}$, C.~W.~Wenzel$^{3}$, U.~Wiedner$^{3}$, G.~Wilkinson$^{69}$, M.~Wolke$^{75}$, L.~Wollenberg$^{3}$, C.~Wu$^{39}$, J.~F.~Wu$^{1,8}$, L.~H.~Wu$^{1}$, L.~J.~Wu$^{1,63}$, X.~Wu$^{12,f}$, X.~H.~Wu$^{34}$, Y.~Wu$^{71}$, Y.~H.~Wu$^{55}$, Y.~J.~Wu$^{31}$, Z.~Wu$^{1,58}$, L.~Xia$^{71,58}$, X.~M.~Xian$^{39}$, T.~Xiang$^{46,g}$, D.~Xiao$^{38,j,k}$, G.~Y.~Xiao$^{42}$, S.~Y.~Xiao$^{1}$, Y. ~L.~Xiao$^{12,f}$, Z.~J.~Xiao$^{41}$, C.~Xie$^{42}$, X.~H.~Xie$^{46,g}$, Y.~Xie$^{50}$, Y.~G.~Xie$^{1,58}$, Y.~H.~Xie$^{6}$, Z.~P.~Xie$^{71,58}$, T.~Y.~Xing$^{1,63}$, C.~F.~Xu$^{1,63}$, C.~J.~Xu$^{59}$, G.~F.~Xu$^{1}$, H.~Y.~Xu$^{66}$, Q.~J.~Xu$^{16}$, Q.~N.~Xu$^{30}$, W.~Xu$^{1}$, W.~L.~Xu$^{66}$, X.~P.~Xu$^{55}$, Y.~C.~Xu$^{77}$, Z.~P.~Xu$^{42}$, Z.~S.~Xu$^{63}$, F.~Yan$^{12,f}$, L.~Yan$^{12,f}$, W.~B.~Yan$^{71,58}$, W.~C.~Yan$^{80}$, X.~Q.~Yan$^{1}$, H.~J.~Yang$^{51,e}$, H.~L.~Yang$^{34}$, H.~X.~Yang$^{1}$, Tao~Yang$^{1}$, Y.~Yang$^{12,f}$, Y.~F.~Yang$^{43}$, Y.~X.~Yang$^{1,63}$, Yifan~Yang$^{1,63}$, Z.~W.~Yang$^{38,j,k}$, Z.~P.~Yao$^{50}$, M.~Ye$^{1,58}$, M.~H.~Ye$^{8}$, J.~H.~Yin$^{1}$, Z.~Y.~You$^{59}$, B.~X.~Yu$^{1,58,63}$, C.~X.~Yu$^{43}$, G.~Yu$^{1,63}$, J.~S.~Yu$^{25,h}$, T.~Yu$^{72}$, X.~D.~Yu$^{46,g}$, C.~Z.~Yuan$^{1,63}$, L.~Yuan$^{2}$, S.~C.~Yuan$^{1}$, Y.~Yuan$^{1,63}$, Z.~Y.~Yuan$^{59}$, C.~X.~Yue$^{39}$, A.~A.~Zafar$^{73}$, F.~R.~Zeng$^{50}$, S.~H. ~Zeng$^{72}$, X.~Zeng$^{12,f}$, Y.~Zeng$^{25,h}$, Y.~J.~Zeng$^{1,63}$, X.~Y.~Zhai$^{34}$, Y.~C.~Zhai$^{50}$, Y.~H.~Zhan$^{59}$, A.~Q.~Zhang$^{1,63}$, B.~L.~Zhang$^{1,63}$, B.~X.~Zhang$^{1}$, D.~H.~Zhang$^{43}$, G.~Y.~Zhang$^{19}$, H.~Zhang$^{71}$, H.~C.~Zhang$^{1,58,63}$, H.~H.~Zhang$^{59}$, H.~H.~Zhang$^{34}$, H.~Q.~Zhang$^{1,58,63}$, H.~Y.~Zhang$^{1,58}$, J.~Zhang$^{80}$, J.~Zhang$^{59}$, J.~J.~Zhang$^{52}$, J.~L.~Zhang$^{20}$, J.~Q.~Zhang$^{41}$, J.~W.~Zhang$^{1,58,63}$, J.~X.~Zhang$^{38,j,k}$, J.~Y.~Zhang$^{1}$, J.~Z.~Zhang$^{1,63}$, Jianyu~Zhang$^{63}$, L.~M.~Zhang$^{61}$, L.~Q.~Zhang$^{59}$, Lei~Zhang$^{42}$, P.~Zhang$^{1,63}$, Q.~Y.~~Zhang$^{39,80}$, Shuihan~Zhang$^{1,63}$, Shulei~Zhang$^{25,h}$, X.~D.~Zhang$^{45}$, X.~M.~Zhang$^{1}$, X.~Y.~Zhang$^{50}$, Y.~Zhang$^{69}$, Y. ~Zhang$^{72}$, Y. ~T.~Zhang$^{80}$, Y.~H.~Zhang$^{1,58}$, Yan~Zhang$^{71,58}$, Yao~Zhang$^{1}$, Z.~D.~Zhang$^{1}$, Z.~H.~Zhang$^{1}$, Z.~L.~Zhang$^{34}$, Z.~Y.~Zhang$^{43}$, Z.~Y.~Zhang$^{76}$, G.~Zhao$^{1}$, J.~Y.~Zhao$^{1,63}$, J.~Z.~Zhao$^{1,58}$, Lei~Zhao$^{71,58}$, Ling~Zhao$^{1}$, M.~G.~Zhao$^{43}$, R.~P.~Zhao$^{63}$, S.~J.~Zhao$^{80}$, Y.~B.~Zhao$^{1,58}$, Y.~X.~Zhao$^{31,63}$, Z.~G.~Zhao$^{71,58}$, A.~Zhemchugov$^{36,a}$, B.~Zheng$^{72}$, J.~P.~Zheng$^{1,58}$, W.~J.~Zheng$^{1,63}$, Y.~H.~Zheng$^{63}$, B.~Zhong$^{41}$, X.~Zhong$^{59}$, H. ~Zhou$^{50}$, L.~P.~Zhou$^{1,63}$, X.~Zhou$^{76}$, X.~K.~Zhou$^{6}$, X.~R.~Zhou$^{71,58}$, X.~Y.~Zhou$^{39}$, Y.~Z.~Zhou$^{12,f}$, J.~Zhu$^{43}$, K.~Zhu$^{1}$, K.~J.~Zhu$^{1,58,63}$, L.~Zhu$^{34}$, L.~X.~Zhu$^{63}$, S.~H.~Zhu$^{70}$, S.~Q.~Zhu$^{42}$, T.~J.~Zhu$^{12,f}$, W.~J.~Zhu$^{12,f}$, Y.~C.~Zhu$^{71,58}$, Z.~A.~Zhu$^{1,63}$, J.~H.~Zou$^{1}$, J.~Zu$^{71,58}$
\\
\vspace{0.2cm}
(BESIII Collaboration)\\
\vspace{0.2cm} {\it
$^{1}$ Institute of High Energy Physics, Beijing 100049, People's Republic of China\\
$^{2}$ Beihang University, Beijing 100191, People's Republic of China\\
$^{3}$ Bochum  Ruhr-University, D-44780 Bochum, Germany\\
$^{4}$ Budker Institute of Nuclear Physics SB RAS (BINP), Novosibirsk 630090, Russia\\
$^{5}$ Carnegie Mellon University, Pittsburgh, Pennsylvania 15213, USA\\
$^{6}$ Central China Normal University, Wuhan 430079, People's Republic of China\\
$^{7}$ Central South University, Changsha 410083, People's Republic of China\\
$^{8}$ China Center of Advanced Science and Technology, Beijing 100190, People's Republic of China\\
$^{9}$ China University of Geosciences, Wuhan 430074, People's Republic of China\\
$^{10}$ Chung-Ang University, Seoul, 06974, Republic of Korea\\
$^{11}$ COMSATS University Islamabad, Lahore Campus, Defence Road, Off Raiwind Road, 54000 Lahore, Pakistan\\
$^{12}$ Fudan University, Shanghai 200433, People's Republic of China\\
$^{13}$ GSI Helmholtzcentre for Heavy Ion Research GmbH, D-64291 Darmstadt, Germany\\
$^{14}$ Guangxi Normal University, Guilin 541004, People's Republic of China\\
$^{15}$ Guangxi University, Nanning 530004, People's Republic of China\\
$^{16}$ Hangzhou Normal University, Hangzhou 310036, People's Republic of China\\
$^{17}$ Hebei University, Baoding 071002, People's Republic of China\\
$^{18}$ Helmholtz Institute Mainz, Staudinger Weg 18, D-55099 Mainz, Germany\\
$^{19}$ Henan Normal University, Xinxiang 453007, People's Republic of China\\
$^{20}$ Henan University, Kaifeng 475004, People's Republic of China\\
$^{21}$ Henan University of Science and Technology, Luoyang 471003, People's Republic of China\\
$^{22}$ Henan University of Technology, Zhengzhou 450001, People's Republic of China\\
$^{23}$ Huangshan College, Huangshan  245000, People's Republic of China\\
$^{24}$ Hunan Normal University, Changsha 410081, People's Republic of China\\
$^{25}$ Hunan University, Changsha 410082, People's Republic of China\\
$^{26}$ Indian Institute of Technology Madras, Chennai 600036, India\\
$^{27}$ Indiana University, Bloomington, Indiana 47405, USA\\
$^{28}$ INFN Laboratori Nazionali di Frascati , (A)INFN Laboratori Nazionali di Frascati, I-00044, Frascati, Italy; (B)INFN Sezione di  Perugia, I-06100, Perugia, Italy; (C)University of Perugia, I-06100, Perugia, Italy\\
$^{29}$ INFN Sezione di Ferrara, (A)INFN Sezione di Ferrara, I-44122, Ferrara, Italy; (B)University of Ferrara,  I-44122, Ferrara, Italy\\
$^{30}$ Inner Mongolia University, Hohhot 010021, People's Republic of China\\
$^{31}$ Institute of Modern Physics, Lanzhou 730000, People's Republic of China\\
$^{32}$ Institute of Physics and Technology, Peace Avenue 54B, Ulaanbaatar 13330, Mongolia\\
$^{33}$ Instituto de Alta Investigaci\'on, Universidad de Tarapac\'a, Casilla 7D, Arica 1000000, Chile\\
$^{34}$ Jilin University, Changchun 130012, People's Republic of China\\
$^{35}$ Johannes Gutenberg University of Mainz, Johann-Joachim-Becher-Weg 45, D-55099 Mainz, Germany\\
$^{36}$ Joint Institute for Nuclear Research, 141980 Dubna, Moscow region, Russia\\
$^{37}$ Justus-Liebig-Universitaet Giessen, II. Physikalisches Institut, Heinrich-Buff-Ring 16, D-35392 Giessen, Germany\\
$^{38}$ Lanzhou University, Lanzhou 730000, People's Republic of China\\
$^{39}$ Liaoning Normal University, Dalian 116029, People's Republic of China\\
$^{40}$ Liaoning University, Shenyang 110036, People's Republic of China\\
$^{41}$ Nanjing Normal University, Nanjing 210023, People's Republic of China\\
$^{42}$ Nanjing University, Nanjing 210093, People's Republic of China\\
$^{43}$ Nankai University, Tianjin 300071, People's Republic of China\\
$^{44}$ National Centre for Nuclear Research, Warsaw 02-093, Poland\\
$^{45}$ North China Electric Power University, Beijing 102206, People's Republic of China\\
$^{46}$ Peking University, Beijing 100871, People's Republic of China\\
$^{47}$ Qufu Normal University, Qufu 273165, People's Republic of China\\
$^{48}$ Renmin University of China, Beijing 100872, People's Republic of China\\
$^{49}$ Shandong Normal University, Jinan 250014, People's Republic of China\\
$^{50}$ Shandong University, Jinan 250100, People's Republic of China\\
$^{51}$ Shanghai Jiao Tong University, Shanghai 200240,  People's Republic of China\\
$^{52}$ Shanxi Normal University, Linfen 041004, People's Republic of China\\
$^{53}$ Shanxi University, Taiyuan 030006, People's Republic of China\\
$^{54}$ Sichuan University, Chengdu 610064, People's Republic of China\\
$^{55}$ Soochow University, Suzhou 215006, People's Republic of China\\
$^{56}$ South China Normal University, Guangzhou 510006, People's Republic of China\\
$^{57}$ Southeast University, Nanjing 211100, People's Republic of China\\
$^{58}$ State Key Laboratory of Particle Detection and Electronics, Beijing 100049, Hefei 230026, People's Republic of China\\
$^{59}$ Sun Yat-Sen University, Guangzhou 510275, People's Republic of China\\
$^{60}$ Suranaree University of Technology, University Avenue 111, Nakhon Ratchasima 30000, Thailand\\
$^{61}$ Tsinghua University, Beijing 100084, People's Republic of China\\
$^{62}$ Turkish Accelerator Center Particle Factory Group, (A)Istinye University, 34010, Istanbul, Turkey; (B)Near East University, Nicosia, North Cyprus, 99138, Mersin 10, Turkey\\
$^{63}$ University of Chinese Academy of Sciences, Beijing 100049, People's Republic of China\\
$^{64}$ University of Groningen, NL-9747 AA Groningen, The Netherlands\\
$^{65}$ University of Hawaii, Honolulu, Hawaii 96822, USA\\
$^{66}$ University of Jinan, Jinan 250022, People's Republic of China\\
$^{67}$ University of Manchester, Oxford Road, Manchester, M13 9PL, United Kingdom\\
$^{68}$ University of Muenster, Wilhelm-Klemm-Strasse 9, 48149 Muenster, Germany\\
$^{69}$ University of Oxford, Keble Road, Oxford OX13RH, United Kingdom\\
$^{70}$ University of Science and Technology Liaoning, Anshan 114051, People's Republic of China\\
$^{71}$ University of Science and Technology of China, Hefei 230026, People's Republic of China\\
$^{72}$ University of South China, Hengyang 421001, People's Republic of China\\
$^{73}$ University of the Punjab, Lahore-54590, Pakistan\\
$^{74}$ University of Turin and INFN, (A)University of Turin, I-10125, Turin, Italy; (B)University of Eastern Piedmont, I-15121, Alessandria, Italy; (C)INFN, I-10125, Turin, Italy\\
$^{75}$ Uppsala University, Box 516, SE-75120 Uppsala, Sweden\\
$^{76}$ Wuhan University, Wuhan 430072, People's Republic of China\\
$^{77}$ Yantai University, Yantai 264005, People's Republic of China\\
$^{78}$ Yunnan University, Kunming 650500, People's Republic of China\\
$^{79}$ Zhejiang University, Hangzhou 310027, People's Republic of China\\
$^{80}$ Zhengzhou University, Zhengzhou 450001, People's Republic of China\\
\vspace{0.2cm}
$^{a}$ Also at the Moscow Institute of Physics and Technology, Moscow 141700, Russia\\
$^{b}$ Also at the Novosibirsk State University, Novosibirsk, 630090, Russia\\
$^{c}$ Also at the NRC "Kurchatov Institute", PNPI, 188300, Gatchina, Russia\\
$^{d}$ Also at Goethe University Frankfurt, 60323 Frankfurt am Main, Germany\\
$^{e}$ Also at Key Laboratory for Particle Physics, Astrophysics and Cosmology, Ministry of Education; Shanghai Key Laboratory for Particle Physics and Cosmology; Institute of Nuclear and Particle Physics, Shanghai 200240, People's Republic of China\\
$^{f}$ Also at Key Laboratory of Nuclear Physics and Ion-beam Application (MOE) and Institute of Modern Physics, Fudan University, Shanghai 200443, People's Republic of China\\
$^{g}$ Also at State Key Laboratory of Nuclear Physics and Technology, Peking University, Beijing 100871, People's Republic of China\\
$^{h}$ Also at School of Physics and Electronics, Hunan University, Changsha 410082, China\\
$^{i}$ Also at Guangdong Provincial Key Laboratory of Nuclear Science, Institute of Quantum Matter, South China Normal University, Guangzhou 510006, China\\
$^{j}$ Also at MOE Frontiers Science Center for Rare Isotopes, Lanzhou University, Lanzhou 730000, People's Republic of China\\
$^{k}$ Also at Lanzhou Center for Theoretical Physics, Lanzhou University, Lanzhou 730000, People's Republic of China\\
$^{l}$ Also at the Department of Mathematical Sciences, IBA, Karachi 75270, Pakistan\\
}
\end{center}
\vspace{0.4cm}
\vspace{0.4cm}
\end{small}
}

\noaffiliation{}

